Result and Congestion Aware Optimal Routing and Partial Offloading in Collaborative Edge Computing

Collaborative edge computing (CEC) is an emerging paradigm where heterogeneous edge devices (stakeholders) collaborate to fulfill computation tasks, such as model training or video processing, by sharing communication and computation resources. Nevertheless, the optimal data/result routing and computation offloading strategy in CEC with arbitrary topology still remains an open problem. In this paper, we formulate a partial-offloading and multi-hop routing model for arbitrarily divisible tasks. Each node individually decides the computation of the received data and the forwarding of data/result traffic. In contrast to most existing works, our model applies to tasks with non-negligible result size, and enables separable data sources and result destinations. We propose a network-wide cost minimization problem with congestion-aware cost to jointly optimize routing and computation offloading. This problem covers various performance metrics and constraints, such as average queueing delay with limited processor capacity. Although the problem is non-convex, we provide non-trivial necessary and sufficient conditions for the global-optimal solution, and devise a fully distributed algorithm that converges to the optimum in polynomial time, allows asynchronous individual updating, and is adaptive to changes in network topology or task pattern. Numerical evaluation shows that our proposed method significantly outperforms other baseline algorithms in multiple network instances, especially in congested scenarios.

==> JointOptimization.tex <==
\section{Joint Routing and Offloading Optimization} \label{Section:Optmize}

   
  In this paper, we aim at minimizing the overall cost of mobile edges and devices for both communication and computation, presented as follows,
\begin{align}
    \min_{\boldsymbol{\phi}} \quad & D = \sum_{(i,j) \in E}D_{ij}(F_{ij}) + \sum_{i \in V} C_i(\boldsymbol{G}_i) \label{JointProblem_nodebased}
    \\ \text{such that} \quad & \text{(\ref{ti-}) to (\ref{FlowConservation2.2}) hold} \nonumber
   % \\ & \phi_{ij}^-(d,m) \geq 0, \quad \forall i \in V, (d,m) \in S, j \in \left\{0\right\} \cup V \nonumber
   % \\ & \phi_{ij}^+(d,m) \geq 0, \quad \forall i \in V, (d,m) \in S, j \in V \nonumber
\end{align}
Note that problem (\ref{JointProblem_nodebased}) is not necessary convex in $\boldsymbol{\phi}^-$ and $\boldsymbol{\phi}^+$. %We will first study the case $b = 0$ and provide a global solution, then discuss the general case $b \geq 0$.  %and is NP-hard when $b > 0$, since it contains a general $\ell^0$ norm minimization problem as reduced case.
{\color{blue} Complexity analysis? Relation to flow model problem?}

{\color{blue} Should we mention the isolated looping problem as in \cite{gallager1977minimum} and mention our algorithm can prevent it?}

==> Outline.tex <==
\begin{itemize}
   
\item {Abstract Keyword (0.25 pg)}

 \item {Introduction (1.25 pg)}
\begin{itemize}
    \item Intro of edge computing
    \item Intro of collaborative edge computing (CEC)
    \item Intro of this work
    \item Comparisons to related works
\end{itemize}
 \item {Network routing and computation model(1.75 pg)}

\begin{itemize}
\item
Graph
\begin{itemize}
    \item DAG, set of nodes and links
    \item out-going and in-going neighbors
\end{itemize}

\item
Tasks
\begin{itemize}
    \item pair $(d,m)$
    \item multi-commodity
    \item input rate $r_i(d,m)$
\end{itemize}

\item
Routing/offloading scheme
\begin{itemize}
    \item data and result flow $f^-,f^+$, computation flow $g$
    \item data-result convert $a_m$, examples
    \item node flow $t^-,t^+$
    \item variable $\phi$, flow conservation
\end{itemize}

\item 
Computation and Communication cost
\begin{itemize}
    \item link flow $F_{ij}$ and node compute amount $\boldsymbol{G}_i$
    \item cost $D_{ij}$ and $C_i$
    \item justify model equivalence with other papers, by example
\end{itemize}

\end{itemize}

 \item {Optimization problem formulation (merge to model section)}
\begin{itemize}
    \item Joint problem
    \item Non-convexity
\end{itemize}

 \item {Optimality Conditions (1 pg)}
\begin{itemize}
\item Overview: although non-convex, we will propose a non-trivial sufficient condition
\item Expression of partial derivatives ($\frac{\partial D}{\partial r_i}$ and $\frac{\partial D}{\partial \phi}$)
\item Lagrangian, Lemma for Necessary condition
\item Example for non-sufficiency, modification
\item Sufficient condition theorem
\item Example (previous) with sufficient condition
\end{itemize}

 \item {Algorithm (1.75 pg)}
 \begin{itemize}
     \item Overview: a scaled gradient projection algorithm that converges to sufficient condition
     \item Overview: variable updating formula
     \item elements needed in algorithm
     \begin{itemize}
         \item loop-free property
         \item direct estimation of marginals
         \item broadcast protocol
         \item blocked nodes
         \item scaling matrix
     \end{itemize}
     \item initial point
     \item pseudo-code
     \item asynchronous convergence
 \end{itemize}

\item {simulation (1 pg)}
\begin{itemize}
    \item benchmarks (centralized) description
    \begin{itemize}
        \item Optimal Routing, local computation
        \item Optimal Offloading, fixed path (min-hop)
        \item Optimal 2-hop offloading (or other method in literature)
    \end{itemize}
    \item detail setting
\end{itemize}

\item{conclusion 0.25 pg}

\item{reference 0.75 pg}

\end{itemize}
